A brief comment on the similarities of the IR solutions for the ghost propagator DSE in Landau and Coulomb gauges

This brief note is devoted to reconcile the conclusions from a recent analysis of the IR solutions for the ghost propagator Dyson-Schwinger equations in Coulomb gauge with previous studies in Landau gauge.

==> my-headings.tex <==
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{latexsym}
\usepackage{color}
\usepackage{colordvi}
\usepackage{epsfig}
\usepackage{array}
\usepackage{pifont}
\usepackage{axodraw}


\newcommand{\pslash}{p \!\!\!/}
%\newcommand{\xslash}{x \!\!\!/}
\newcommand{\Dslash}{D \!\!\!/}
\newcommand{\nn}{\nonumber}
\newcommand{\beq}{\begin{eqnarray}}
\newcommand{\eeq}{\end{eqnarray}}
\newcommand{\asgen}{\alpha_s}
\newcommand{\asl}{\alpha_s^{{}^{\rm LATT}}}
\newcommand{\as}{\alpha_s{{}^{\rm MOM}}}
\newcommand{\astil}{\alpha_s{{}^{\widetilde{\rm MOM}}}}
\newcommand{\asms}{\alpha_s{{}^{\overline{\rm MS}}}}
\newcommand{\MSB}{\overline{\rm MS}}
\newcommand{\MOM}{\widetilde{\rm MOM}}
\newcommand{\gduems}{g^2_{\overline{\rm MS}}}
\newcommand{\gdue}{g^2_{\widetilde{\rm MOM}}}
\newcommand{\Lam}{\Lambda_{\widetilde{\rm MOM}}}
\newcommand{\Lams}{\Lambda_{\overline{\rm MS}}}
\newcommand{\Lamlatt}{\Lambda_{{}^{\rm LATT}}}
\newcommand{\gev}{{\rm GeV}}
\newcommand{\mev}{{\rm MeV}}
\newcommand{\fm}{\ \rm{fm}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\lwrsim}{\raise0.3ex\hbox{$<$\kern-0.75em\raise-1.1ex\hbox{$\sim$}}}
\newcommand{\etabar}{\overline{\eta}}
\newcommand{\rhom}{\overline{\rho}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Am#1#2#3{\widetilde A_{#1}^{#2}(#3)}
\def\A#1#2#3{A_{#1}^{#2}(#3)}
\def\C2#1#2{({\cal C}_2)_{#1}^{#2}}
\def\glandau#1#2#3{(g_{#1 #2}-\frac{#3_#1 #3_#2}{#3^2})}
\def\glandauM#1#2#3{(g_{#1 #2}-\frac{#3_#1 #3_#2}{-k^2})}
\def\assylarge#1{\begin{array}{c} \rule[0.45cm]{0cm}{0cm} \to \\ #1 >> 1 
                 \end{array}}
\def\eq#1{Eq.~(\ref{#1})}
\def\altura#1{\rule[0cm]{0cm}{#1cm}}
%%%%%%%%% Defining Feynman rules
\def\PGhost#1#2#3{i\frac{\delta^{#1 #2}}{{#3}^2}}
\def\VGhostGluon#1#2#3#4#5{-g f^{#1 #2 #3} {#5}_{#4}}
\def\PGluon#1#2#3#4#5{-i \frac{\delta^{#1 #2}}{(#5)^2} g^{\perp}_{#3 #4}(#5)}
\def\VThreeGluon#1#2#3#4#5#6#7#8#9{-g f^{#1 #2 #3} 
    \left( g_{#5 #6} (#8-(#9))_{#4} 
         + g_{#6 #4} (#9-(#7))_{#5} 
	 + g_{#4 #5} (#7-(#8))_{#6} \right)}
\def\condGluon#1#2#3#4{\frac 1 2 \delta_{#1 #2} g^{#3 #4}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\appsection}[1]{
%\renewcommand{\thesection}{Appendix~\Alph{section}}
%\section{#1}
%\renewcommand{\thesection}{\Alph{section}}}

%\newcommand{\ewxy}[2]{\setlength{\epsfxsize}{#2}\epsfbox[-40 60 640590]{#1}}
\def\jhep#1#2#3{J. High Energy Phys. {\bf #1} (#2) #3}
\def\prd#1#2#3{Phys.\ Rev.\ {\bf D#1} (#2) #3}
\def\npb#1#2#3{Nucl.\ Phys.\ {\bf B#1} (#2) #3}
\def\plb#1#2#3{Phys.\ Lett.\ {\bf B#1} (#2) #3}
\def\ap#1#2#3{Ann.\ Phys.\ (NY) #1 (19#3) #2}
\def\ar#1#2#3{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ #1 (19#3) #2}
\def\cav#1{Cambridge preprint Cavendish--HEP--#1}
\def\cpc#1#2#3{Computer Phys.\ Comm.\ #1 (19#3) #2}
\def\ib#1#2#3{ibid.\ #1 (19#3) #2}
\def\np#1#2#3{Nucl.\ Phys.\ B#1 (19#3) #2}
\def\pl#1#2#3{Phys.\ Lett.\ #1B (19#3) #2}
\def\pr#1#2#3{Phys.\ Rev.\ D #1 (19#3) #2}
\def\prep#1#2#3{Phys.\ Rep.\ #1 (19#3) #2}
\def\prl#1#2#3{Phys.\ Rev.\ Lett.\ #1 (19#3) #2}
\def\rmp#1#2#3{Rev.\ Mod.\ Phys.\ #1 (19#3) #2}
\def\sj#1#2#3{Sov.\ J.\ Nucl.\ Phys.\ #1 (19#3) #2}
\def\zpc#1#2#3{Z.\ Phys.\ {\bf C#1} (#2) #3}
\def\xslash#1{#1 \!\!\!/}
\def\fig#1{Fig. \ref{#1}}

